Holmes-VAU: Towards Long-term Video Anomaly Understanding at Any Granularity

How can we enable models to comprehend video anomalies occurring over varying temporal scales and contexts? Traditional Video Anomaly Understanding (VAU) methods focus on frame-level anomaly prediction, often missing the interpretability of complex and diverse real-world anomalies. Recent multimodal approaches leverage visual and textual data but lack hierarchical annotations that capture both short-term and long-term anomalies. To address this challenge, we introduce HIVAU-70k, a large-scale benchmark for hierarchical video anomaly understanding across any granularity. We develop a semi-automated annotation engine that efficiently scales high-quality annotations by combining manual video segmentation with recursive free-text annotation using large language models (LLMs). This results in over 70,000 multi-granular annotations organized at clip-level, event-level, and video-level segments. For efficient anomaly detection in long videos, we propose the Anomaly-focused Temporal Sampler (ATS). ATS integrates an anomaly scorer with a density-aware sampler to adaptively select frames based on anomaly scores, ensuring that the multimodal LLM concentrates on anomaly-rich regions, which significantly enhances both efficiency and accuracy. Extensive experiments demonstrate that our hierarchical instruction data markedly improves anomaly comprehension. The integrated ATS and visual-language model outperform traditional methods in processing long videos. Our benchmark and model are publicly available at https://github.com/pipixin321/HolmesVAU.

==> figs/teaser.tex <==
\includegraphics[width=\textwidth]{figs/fig_teaser.pdf}\setlength{\abovecaptionskip}{0.1cm}
\captionof{figure}{
\textbf{Motivation}. \textbf{Left}: Existing datasets lack the hierarchical structure to capture transient and sustained anomalies across varying temporal scales. Our \textit{\textbf{HIVAU-70k}} dataset addresses this by providing multi-granularity annotations—clip, event, and video levels—that enable detailed anomaly analysis in complex real-world scenarios. \textbf{Right}: Inspired by Sherlock Holmes’s knack for zeroing in on critical details, our \textbf{\textit{Holmes-VAU}} method integrates an Anomaly-focused Temporal Sampler with a multi-modal LLM, directing model attention to anomaly-rich segments, which enables models to decode complex, long-term video anomalies efficiently. 
}
\vspace{-6mm}
\label{fig:motivation}

==> tables/datasets_statistics.tex <==
\begin{table}[h!]
\centering
\caption{\textbf{Datasets Statistics}.}
\label{tab:dataset_statistic}
\setlength{\tabcolsep}{4pt}
\begin{tabular}{l|cccc}
\toprule
Dataset & \#Videos & Annotation Type  & \#Queries & Avg word  \\
\midrule
CHUK Avenue &37 &None &N/A &N/A \\
ShanghaiTech &437 &None/video label &N/A &N/A \\
UCF-Crime~\cite{ucf} & 1,610 & video label &N/A & N/A  \\
XD-Violence~\cite{xdviolence} & 4,754 & video label &N/A & N/A \\
UCA~\cite{yuan2023surveillance} & 1,854 & segment caption & 23,542 & 20.15  \\
\midrule
\textbf{VAD-Instruct50k (Ours)}  & \textbf{5,547} & \textbf{single-frame\&segment instruction} & \textbf{51,567} & \textbf{44.83}  \\
\bottomrule
\end{tabular}
% }

\end{table}
